AutoShape: Real-Time Shape-Aware Monocular 3D Object Detection

Existing deep learning-based approaches for monocular 3D object detection in autonomous driving often model the object as a rotated 3D cuboid while the object's geometric shape has been ignored. In this work, we propose an approach for incorporating the shape-aware 2D/3D constraints into the 3D detection framework. Specifically, we employ the deep neural network to learn distinguished 2D keypoints in the 2D image domain and regress their corresponding 3D coordinates in the local 3D object coordinate first. Then the 2D/3D geometric constraints are built by these correspondences for each object to boost the detection performance. For generating the ground truth of 2D/3D keypoints, an automatic model-fitting approach has been proposed by fitting the deformed 3D object model and the object mask in the 2D image. The proposed framework has been verified on the public KITTI dataset and the experimental results demonstrate that by using additional geometrical constraints the detection performance has been significantly improved as compared to the baseline method. More importantly, the proposed framework achieves state-of-the-art performance with real time. Data and code will be available at https://github.com/zongdai/AutoShape

==> Files/01_introduction_by_zongdai.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Perceiving 3D shapes and poses of surrounding obstacles is an essential task in autonomous driving (AD) perception systems. The accuracy and speed performance of 3D objection detection is critically important for the following motion planning and control modules in AD. Many 3D object detectors have been proposed, mainly for depth sensors such as LiDAR or stereo cameras, which can provide the distance information of the environments directly. However, LiDAR sensors are expensive and stereo rigs suffer from on-line calibration issues. 
% Therefore, monocular camera based 3D object detection becomes a promising practical direction.

3D object detection is an essential part of perception system of autonomous driving and robotic. The main challenge is to capture object accurate depth information. Most of the existing methods utilize LiDARS which is expensive and fragile. Based on human visual cognition, camera devices could be a desirable alternatives. However camera can not provide depth directly and stereo rigs suffer from on-line calibration issues. Therefore, monocular camera based 3D object detection becomes a promising direction.

To obtain depth from monocular camera, many methods\cite{ku2019monocular, weng2019monocular, ma2019accurate, vianney2019refinedmpl, ma2020rethinking, ding2020learning} use estimated depth map. They often covert depth map to pseudo-LiDAR or regard depth map as convolutions guider. However, heavy computation burden is one main bottleneck of such two-stage approaches. To improve the efficiency, many image-based methods \cite{liu2020smoke, zhou2020iafa, li2020rtm3d, 2009.00764} have been proposed and achieved promising results. \cite{liu2020smoke, zhou2019objects} use 1 center point and regress depth directly. However the center depth is harder to regress then surface. To address these challenges, geometric constraints are widely used in these methods. \cite{li2020rtm3d, 2009.00764} use 8 corners and 1 center as 2D keypoints and regress object dimension to build 2D-3D geometric constraints to reason object location. Through these methods achieve promising performance on accuracy and speed, the corners have non-real context meanings and the constraint constructed by 9 points is weak and not robust.

To explore more meaningful geometric constraints, an idea strategy is to match each object in image with an exactly 3D model and pose. Then a set of geometric constraints are naturally established. Except ApolloCar3D\cite{song2019apollocar3d}, none dataset provides such annotation, because it is labor expensive.

In order to address the above problems, we propose AutoShape, a novel monocular 3D object detection framework that enables to construct stronger shape-aware geometric constraints from object 3D shape and keep both accurate and efficiency in 3D detection inference. Our framework consists of two main components: 1) a 3D shape auto-labeler which optimizes a parameterized 3D shape to match an object and 2) a single stage monocular 3D detection network. As shown in Fig \ref{Fig:Teaser}. AutoShape automatically aligns object with a 3D model to construct shape-aware geometric constraints to boost the 3D detection performance. More specifically, our network learns to regress 2D/3D keypoints provided by our 3D shape auto-labeler and exerts a geometric reasoning to predict accurate object location. 




% which takes initial pose, Lidar point cloud and instance mask as input to

% 2)direct regress object center depth\cite{liu2020smoke, zhou2020iafa} and 3)geometric constraints solver\cite{brazil2019m3d, li2020rtm3d, 2009.00764}. Estimated depth map often rely on extra stand alone network and is sensitive to camera parameters and scene content. Geometric and semantic constraint 



%and many impressive have been proposed such as CenterNet \cite{zhou2019objects}, SMOKE \cite{liu2020smoke}, etc.
%3D object detection is an essential part of perception system of autonomous driving and robotic. The main challenge is to capture object accurate depth information. Most of the existing methods utilize LiDARS[xxx] which is expensive and fragile. Based on human visual cognition, camera devices could be a desirable alternatives. However camera can not provide depth directly, how to explore geometric and semantic cue to recover location still remains largely unsolved.
% The main challenge for monocular-based approaches is to obtain accurate depth information. In general, depth estimation from a single image without any prior information is a challenging problem and recent many deep learning-based approaches achieve promising results \cite{godard2019digging}. With the estimated depth map, pseudo LiDAR point cloud can be reconstructed via pre-calibrated intrinsic camera parameters and 3D detectors designed for LiDAR point cloud can be applied directly on pseudo LiDAR point cloud \cite{qian2020end} \cite{vianney2019refinedmpl}. Furthermore, \cite{qian2020end} integrate the depth estimation and 3D object detection network together following an end-to-end manner. However, heavy computation burden is one main bottleneck of such two-stage approaches. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
% \centering
% \includegraphics[width=0.98\linewidth]{images/teaser.pdf}
% \caption{(a): Center point + 8 Bbox corners are commonly used in \cite{2009.00764, li2020rtm3d} for providing geometrical constraints, however, their projections on the 2D image share very weak structure meanings. (b) displays an example of alignment result with our proposed 3D shape-guided auto-labeling algorithm. (c) shows the selected shape-aware key-points for the proposed 3D object detection framework where the 2D/3D correspondences are shown in the left bottom and right bottom respectively.
% %Current geometric constraint method \cite{2009.00764, li2020rtm3d} only use few keypoints for 3D localization(a). We present a autolabeler for 3D shape assignment(b), which provides a set of 2D-3D shape points to build geometric constraint(c).
% }
% \label{Fig:Teaser}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% To improve the efficiency, many direct regression-based approaches have been proposed (\eg, SMOKE~\cite{liu2020smoke}, RTM3D~\cite{li2020rtm3d}.) and achieved promising results. By representing the object as one center point, the object detection task is formulated as key-points detection and its corresponding attributes (\eg, size, offsets, orientation, depth, \etc) regression. With this compact representation, the computation speed of this kind of approach can reach 30 fps (frame per second). However, the drawback is also obvious. One center point \cite{zhou2019objects, liu2020smoke} representation ignores the detailed shape of the object and results in location ambiguity if its projected center point is on another object's surface due to occlusion \cite{zhou2020iafa}. 
% %or 9 points (one center point + 8 corners) and object detection has been transferred as a problem of key-points detection and its corresponding attributes (e.g., size, offsets, depth, etc.) regression. With this compact representation, the computation speed of this kind of approach can reach about 30 fps (frame per second). 
% %Although the above representation is very simple and effective for the deep-learning-based framework, the drawbacks are also obvious. Represent an object as only one point \cite{zhou2019objects, liu2020smoke} will ignore the detailed shape of different objects and this results in location ambiguity under occlusion situations \cite{zhou2020iafa}. 
% To alleviate this ambiguity, other geometrical constraints have been employed to improve the performance. RTM3D~\cite{li2020rtm3d} adds 8 more key-points as additional constraints which are defined as the projected 2d location of the 3D bounding box's corners. However, these key-points have non-real context meanings and their 2D locations vary differently with the changing of the camera view-point, even the object's orientation. As shown in Fig.~\ref{Fig:Teaser}, some key-points are on the ground and some are on the sky or trees. This makes the key-points classification network extremely difficult to distinguish the key-points or other image pixels.

% In this paper, we propose a novel approach to learn the meaningful key-points on the object surface and then use them as additional geometrical constraints for 3D object detection. Specifically, we design a CAD model-based object shape annotation pipeline first to generate the 2D/3D correspondences for each object. Then, the center point plus several distinguished key-points are learned from the deep neural network. Based on these key-points and other regressed objects' attributes (\eg, orientation angle, object dimension \etc), the object's 3D bounding box can be solved with linear equations. Our framework can be trained in an end-to-end manner. Our contributions include:
% \begin{enumerate}
% \item We proposed a shape-guided 3d object detection framework, which adds specific key-points constraints on 2D/3D regression. 
% \item We present a new method to automatically generate 2D/3D correspondence for the KITTI dataset. The generated 2D/3D data will be made public for the community.
% \item The effectiveness of our approach has been verified on the public KITTI dataset and achieved SOTA performance for both the 2D BEV and 3D object detection tasks. More importantly, the proposed framework can achieve $25$ fps, which can be directly used in the real applications. 
% \end{enumerate}

%To obtain depth from monocular camera, current methods can be divided into two streams as estimated depth map guided and geometric solver. Estimated depth map often rely on extra stand alone network and is sensitive to camera parameters and scene content. Geometric and semantic constraint, due to lack of diverse 3d shape alignment, often have few evidence to use. [xxx] only use 8 corners and 1 center of object, which carry limited geometric information. Recently, AplloCar3D[] provides 3D model aligned which improve the understanding of AD scene. However, labeling such dataset is laborious and laborious. Moreover, this labeling task is intricacy, including 3D model selection and 6DoF pose adjusting to ensure the accuracy from both 2D appearance and 3D location.

% 有一篇文章也是讲自动标注的，不知道该如何提及 "Autolabeling 3D Objects with Differentiable Rendering of SDF Shape Priors"

%In this paper, we present an automatic annotation method to assign 3D shape to existing labeled instance and an efficient and accurate monocular 3D detection method which utilize more geometry and semantic information.

%Our autolabeling approach utilizes 3D deformable model[permo] to represent various vehicle shape and adopt "render-and-compare" to optimize shape and pose parameters by a differentiable renderer. Given 2D instance mask, initial pose and sparse point cloud, our method could recover accurate 3D shape for 3D bbox instance. Current AD datasets, such as Kitti[] and Nuscene[], can be extended automatically.   




